Drop, Swap, and Generate: A Self-Supervised Approach for Generating Neural Activity

Meaningful and simplified representations of neural activity can yield insights into how and what information is being processed within a neural circuit. However, without labels, finding representations that reveal the link between the brain and behavior can be challenging. Here, we introduce a novel unsupervised approach for learning disentangled representations of neural activity called Swap-VAE. Our approach combines a generative modeling framework with an instance-specific alignment loss that tries to maximize the representational similarity between transformed views of the input (brain state). These transformed (or augmented) views are created by dropping out neurons and jittering samples in time, which intuitively should lead the network to a representation that maintains both temporal consistency and invariance to the specific neurons used to represent the neural state. Through evaluations on both synthetic data and neural recordings from hundreds of neurons in different primate brains, we show that it is possible to build representations that disentangle neural datasets along relevant latent dimensions linked to behavior.

==> Attempts.tex <==


\section{Attempts}

This section is temporarily put here to organize the logic of designing experiments.


\subsection{Using InfoGAN to generate views}

\paragraph{Good results on Mnist}

Although the classification accuracy did not change much, the latent space showed much better separability on digit class \footnote{It would be good if there is another evaluation method, like the uniformity and alignment.}. Also, when visualizing the rotation angles, the rotation angles showed better `direction' (regression results), where the latent space of BYOL separates heavily rotated images and barely rotated images, while GV-BYOL separates clockwise rotation and counter-clockwise rotation \footnote{It would be good if there is also a quantitative method.}.

We can surmise that: generative models typically organize the latent representation such that the change of a latent variable has some interpretability, which sometimes makes sense e.g. color change, rotation angle, but sometimes does not make sense e.g. change from a cat to a tree. This property of generative models (organizing latent variables so that we can interpret its change along a direction) gives contrastive methods more interpretability.

\paragraph{Issues of InfoGAN}

Although the previous experiments showed promising sign of using generative views to perform contrastive learning, there are two non-negligible issues. 

1) InfoGANs generally would have a hard time generalizing on more complex datasets, e.g. Cifar. If the aim of the paper is to improve contrastive learning performance, Cifar level evaluation is necessary. Note that it is unclear if it is the problem of the Cifar dataset (lower resolution but high complexity) or if it is the problem of InfoGAN.


2) The computational resources required for training both GAN and contrastive model are high. This also would challenge the motivation of the paper.

Computational resources: Training a (GAN + BYOL) coarsely equals training 3 BYOLs (1 discriminator, 1 generator, 1 BYOL). Merging the GAN with BYOL still equalas training 2 BYOLs (1 generator, 1 BYOL/discriminator). 

Challenge of motivation: Does it make sense to train 3 or 2 BYOLs \emph{just} to get rid of the hand-selection of augmentations? -- How to make the motivation `stronger'?

\subsection{Solution 1: Use an instance specific GAN}

\paragraph{StyleGAN and style transfer}

Image generation in InfoGAN is based on learning the distribution of the whole dataset. As an alternative, StyleGAN generates images based on the distribution of a given image, which is easier for the model and thus the image quality is generally better with a possible sacrifice of diversity.

% \paragraph{Using StyleGAN to generate views}

\subsection{Solution 2: Generate latents instead of views}

Generating latent representation directly is much more efficient than generating views directly.


\subsection{Novelty 1: Use a private latent space}

Notations:
\begin{itemize}
    \item Image space: $\mathbf{x} \in \mathcal{D}$.
    \item Latent space: $\mathbf{v} \in \mathcal{V}$. This latent space is the latent space that is commonly used to perform linear classification evaluation.
    \item Online networks: Encoder $f_\theta$, projector $g_\theta$, predictor $p_\theta$.
    \item Target networks: Encoder $f_\xi$, projector $g_\xi$, which are not trained but are moving average of online networks.
    \item $f_\theta(\mathbf{x}) = \mathbf{v}$, which $\mathcal{V}$ is the latent space that is commonly used to do linear evaluation.
    \item Generator network: $\phi({\bf v}_c, {\bf v}_p)$
    %\item BYOL loss is an $l_2$ loss function that minimize the distance between $p_\theta(g_\theta(f_\theta(\mathbf{x}_{1})))$ and $g_\xi(f_\xi(\mathbf{x}_{2}))$.\eva{not entirely true since we are splitting variables, lets write it out rather than in bullets}
\end{itemize}


Assume that $\mathbf{v} \in \mathcal{V}$ consists of two parts, a private space and common space $\mathbf{v}^{p}$ and $\mathbf{v}^{c}$ respectively. The common space is regularized \eva{not just regularized i guess... controlled} by a L2-loss (as in BYOL), where all data augmentations related information are `collapsed' and visual semantics are preserved. On the other hand, the private space is `freed' to store other information related to the reconstruction task that might not be useful when building in specific invariances into the common space (imposed by specific choices of data augmentation (DA)). The private space can be used to generate images, which would regularize it to contain different but (hopefully) interpretable information.

We propose the following algorithm for training a system to solve both objectives in cohesive manner, where both objectives can help one another and facilitate more robust generative models as well as even further separability in downstream tasks of interest in representation learning. We want the best of both in one model!

%\paragraph{Reconstruction loss} 


%\begin{equation}
 %   \mathcal{L}_r =  \min_{\phi} \| {\bf x} - \phi( {\bf v}_{c}, {\bf v}_p ) \| + \| {\bf x}' - \phi({\bf v}_{c}', {\bf v}_p' ) \| 
%\end{equation}

\paragraph{Objective function:} 
Let $\widehat{\bf x} = \phi( {\bf v}_{c}, {\bf v}_p )$ denote the reconstruction of $\bf x$ provided by the generator. 
\begin{equation}
\label{eq:main}
     \min_{f, g, p, \phi} \| p_\theta(g_\theta({\bf v}_c)))  - g_\xi({\bf v}_c')) \|_2 + \lambda_1 \| {\bf x} - \phi( {\bf v}_{c}, {\bf v}_p )  \| + \lambda_2 \| {\bf x}' - \phi( {\bf v}_{c}', {\bf v}_p' ) \| 
\end{equation}

\paragraph{Algorithm for training}
\begin{enumerate}
    \item Update dual networks to minimize the overall loss in Equation~\ref{eq:main}.
    \item Update the generator using a content swapping strategy.
\end{enumerate}




% \eva{Is that what you mean? However, I don't know how to train this model by doing this, because the encoder would need BYOL loss and discriminator loss. BYOL loss train encoder/projector/predictor together, discriminator only train encoder. Encoder would be trained twice, which can not be done practically.}

% \eva{The normal way to separate encoder and generator is to train encoder/projector/predictor using only BYOL loss, train the discriminator head using discriminator loss, and train generator using generator loss. However, in this way, the encoder private space in encoder or projector would not be regularized. -- Another way is to train the encoder/projector/predictor using BYOL loss + discriminator loss, and train the generator using generator loss. This way would be ok, but it does not make sense to train the predictor space with a discriminator loss.}


\subsection{New motivation based on Novelty 1: learn augmentation based on augmentation}

Current methods are to maximize the similarity between $x_1$ and $x_2$, where $x_1$ and $x_2$ are two augmented version of image $x$. However, it is not accurate: there is a content part and a style part in the latent space of $x_1$ and $x_2$.

Write the latent space of any image $x_i$ as $[v_{c_i}, v_{p_i}]$, where the $v_{c_i}$ is the content latent and $v_{p_i}$ is the private latent, or to say style latent. For image $x_1$ and $x_2$, we want $v_{c_1} = v_{c_2}$ and $v_{p_1} \neq v_{p_2}$, and also the differences between $v_{p_1}$ and $v_{p_2}$ should reflect the differences between the augmentations applied.

Using $x_1$ and $x_2$, the two augmented versions of images to learn the separation, and thus, by doing interpolation of the style space, we can create new positive views for $x$. 

\rliu{My point is that: our model needs a `highlight'. It is difficult to sell the work if we just say our model can do A and B together. It can be better than all other models in A or B, or it solves a new task C, where in the paper we can write such that C is an important problem.}


An intuitive realization would be using the VAE to reconstruct. However, in VAE the encoder and decoder need to be trained together. Therefore, the only method to train encoder based on VAE would be summing up the BYOL loss with the final reconstruction loss function and backpropergate them together. This method seems not intuitive enough.

Thus, we choose to develop this model based on GAN. However, it is not intuitive and easy to regularize GAN such that the input image correspond to the output image. There are a few ways to do that: 1) use the Adain module in style transfer domain like StyleGAN. 2) use the Unet architecture in pix2pix. 3) use the latent code regularization method like L2 regression such as CycleGAN.

CycleGAN loss operates on the latent space. Thus, we modify the loss function based on that to get the separable representation space. First, we write the original CycleGAN loss as below:
The CycleGAN discriminator is trained by the loss function:
$$
L_{CycleGAN, D} = 0.5* [D(x_{real}, 1) + D(x_{fake}, 0)]
$$
The generator is trained by the loss function:
$$
L_{CycleGAN, G} = D(x_{fake}, 1) + \lambda * MAE(x_{real}, x_{identity}) + \beta * MAE(x_{real}, x_{translated})
$$
Since CycleGAN has a different purpose of designing, the above loss function is difficult to understand, but it can be re-written as our case below:
$$
L_{ours, G} = D(x_{fake}, 1) + \lambda * MAE(x_{real}, G(v_{c, real}, v_{p, real})) + \beta * MAE(x_{real}, G(v_{c, borrowed}, v_{p, real}))
$$



\paragraph{Comparison}

Our model performance.

Original Generator (VAE?) performance.

Original Generator with private space but not BYOL performance.

==> architecture.tex <==

\subsection{Implementation and architecture}

If we use a discriminative loss for our generator, then the losses for each part of the network is as follows.
\begin{equation}
    \begin{aligned}
    \text{Encoder } & \mathcal{L}_{f} = \| z^{\prime} - q(z) \|_2^2 \\
    \text{Generator } & \mathcal{L}_{g} = BCE(x, x^{\prime}) + \| z^{\prime} - q(z) \|_2^2 \\ 
    \text{Discriminator } & \mathcal{L}_{d} = BCE(x, x^{\prime})
    \end{aligned}
\end{equation}

For the generator loss function, the first part of the loss aims to make sure that the generator is learning an image $x^{\prime}$ that aligns the data distribution. The second part ensures that the generated positive view is instance specific given the information $z$, where $z^{\prime} = f(g(z+n))$ should be close enough to $z$. Three networks are trained simultaneously.

\paragraph{Getting rid of the discriminator} - \rliu{To do} The function of the discriminator is to ensure the learned image $x^{\prime}$ is within the distribution of image set of $x$. However, a classifier is not necessary for this. Here we replace the discriminator with some distributional loss. [Wasserstein loss etc]

\paragraph{More intuition} \textbf{How will generator help contrastive net:} GANs can generate diverse views based on the information of one image. This view is beneficial for contrastive learning framework because it provides more diverse views to serve as negative examples and positive examples. \textbf{How will contrastive net help generator:} Generator needs a discriminator to distinguish if the image is within the data distribution. With a contrastive network (or contrastive loss function), GAN can be instance specific. [?] 

KNN in the image space correspond to KNN in the latent space?


% This framework is a combination of GAN and Contrastive Network (BYOL). However, there are two differences. First, the original generator of GAN is conditioned such that it becomes an instance specific generator that generates images depending on the conditional information given. Second, the original contrastive network is changed such that the original "clustering $\Rightarrow$ move-representation" step is changed. The clustering step is no longer dependent on the data augmentation, but depends on the generated datapoints. [TBD]

==> checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerTODO{}
%   \item Did you include the license to the code and datasets? \answerTODO{}
%   \item Did you include the license to the code and datasets? \answerTODO{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See Section \ref{sec:conclusion}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{To our knowledge, this work will have no negative societal impacts.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{After review, a URL to all relevant code and a demo will be included at the beginning of Section \ref{sec:methods}}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Section \ref{sec:experiments}}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{See Appendix \ref{app:implementation}}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Section \ref{subsec:Experiments_on_neural_datasets}}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{After review, a URL to all relevant code and a demo will be included at the beginning of Section \ref{sec:methods}}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> idea-mixup.tex <==


\section{Introduction}

\paragraph{Contributions} a) Our proposed framework provides a domain-agnostic way to perform augmentation in self-supervised learning methods.

b) A generative framework to provide positive and/or negative examples which would train the contrastive model more efficiently and effectively.

\section{Related works}

\paragraph{Clever collapsing}

Current mixing ideas are based on the convex combination of different samples in the image space \cite{zhang2017mixup} or the latent space \cite{verma2019manifold}, and thus provided limited performance [need reference]. [Any work focused on a better collapsing (a learned interpolation)?] [Generative learning in the latent space?] [TBD]

\paragraph{Domain-agnostic augmentation is important}

Augmentation is a key building block of self-supervised learning algorithms. While there are works working on the automated search of augmentations \cite{cubuk2019autoaugment,ho2019population,cubuk2020randaugment}, a list of possible augmentations need to be provided to serve as a search space for the best policy. However, different domains require different augmentations. The augmentations commonly used in image classification domain does not provide best performance boosts to other domains, including vision-related task like object detection \cite{zoph2020learning}, and tasks in other domains like biomedical image classification \cite{pesteie2019adaptive}. Thus, more powerful domain-agnostic augmentation methods are needed in self-supervised learning. 

\paragraph{Latent/Image interpolation for augmentation} 

There are some works performed interpolation in the latent space as data augmentation. The works are extensive under the supervised setting, which can be categorized to two types: a) image space interpolation \cite{zhang2017mixup}, b) latent space interpolation \cite{devries2017dataset,verma2019manifold}. For unsupervised learning and self-supervised learning domain, the works are limited. Based on MoCo, \cite{kalantidis2020hard} performed latent interpolation for negative examples, to help the positive examples learn "harder" negative examples. Based on MoCo as well, \cite{shen2020rethinking} performed image space interpolation to enhance the training space which soften the prediction space boundary. 

\paragraph{Generative learning as augmentation}

There are a lot of papers using generative networks to generate more diverse data points that is used to augment the original dataset. Among many works, \cite{lemley2017smart} developed a generative network that learns the "merge" of two images to enhance the training space.


\section{Methods}

\subsection{Tentative loss function}

\paragraph{Image interpolation}

Images are mixed up like below:
\begin{equation}
\begin{aligned}
    x_1 &= (1- \alpha) x + \alpha r_1 \\
    x_2 &= (1- \alpha) x + \alpha r_2
\end{aligned}
\end{equation}
where $x$ is the main image, $r_1$ and $r_2$ are two random images, $\alpha$ is a random number that is randomly sampled from range $(0, MAX)$. Those two images are feed inside the BYOL loss as below:
\begin{equation}
    \mathcal{L} = \mathcal{L}_{byol} (x_1, x_2)
\end{equation}


\paragraph{Symmetric image interpolation}

[Not tested yet, since image interpolation is not acting better than latent interpolation now] The symmetric merging of the images are like below:
\begin{equation}
\begin{aligned}
    x_1 &= (1- \alpha) x + \alpha r \\
    x_2 &= \alpha x + (1- \alpha) r
\end{aligned}
\end{equation}
where $x$ is the main image, $r$ is a random image, $\alpha$ is a random number that is randomly sampled from range $(0, MAX)$. Those two images are feed inside an edited version of BYOL loss as below:
\begin{equation}
\begin{aligned}
    \mathcal{L} = \mathcal{L}_{byol}^{adjusted} (x, x_1) + \mathcal{L}_{byol}^{adjusted} (r, x_2)
\end{aligned}
\end{equation}
The BYOL loss is adjusted so that it is punishing the percentage of the distance instead of the distance itself. Otherwise, $x$ will be collapsing with all $r$.

\paragraph{Augmentation-assisted latent interpolation/extrapolation}

Here we design a loss function based on augmentation to gain intuition.
Treat the online network (encoder + projector) as function $f$, the target network is $f^'$ with the same architecture but different weights as $f$. Take $x$ from the data and $x_1$ and $x_2$ as two augmented view of $x$. The following operation is done on the projector latent space of both the online network and the target network:
\begin{equation}
\begin{aligned}
    f(view_1) &= (1- \alpha) f(x_1) + \alpha f(x) \\
    f(view_2) &= (1- \alpha) f(x_2) + \alpha f(x)
\end{aligned}
\end{equation}
As stated above, $f^{'}(view_1)$ and $f^{'}(view_2)$ are computed similarly. Then the output of the online encoder is passed inside the predictor $g$, and the BYOL loss is computed based on $L_2(g(f(view_1)), f^{'}(view_2))$ and $L_2(g(f(view_2)), f^{'}(view_1))$.


\section{Experiments}

\subsection{Image Classification}

\subsection{Few-shot unsupervised learning?}

\bibliography{bib/refs_augmentation}
\bibliographystyle{abbrv}


==> possible_direction.tex <==
\section{Possible directions/insights}
\subsection{Enforcing Interpolation Consistency Across Layers}

\subsection{Efficient Way of Using Negative Examples}

Current methods such that SimCLR and MoCo are computational-expensive because they either use a large batch size or a large memory bank to store the negative examples. BYOL shows that one can use only positive examples to construct an effective representation space for learning. However, the latent space of BYOL is highly clustered due to the lack of negative examples. Here, we introduce a method to use negative examples efficiently in BYOL to reduced the clustering effect.

==> text/decoding1.tex <==




\begin{table}[h]
\centering
\caption{Accuracy (in \%) for classification on neural datasets. Here * means that the data is copied from MYOW and is subject to change.}
\label{table: classification}
\begin{tabular}{llcccccc}

            & & supervised & VAE & pi-VAE & BYOL & MYOW & Ours \\\hline
\multirow{2}{*}{Chewie-day1} & acc & 63.29^* & x  & & 63.80^* & 70.41^* & \\ & delta-acc & 63.29^* & x  & & 63.80^* & 70.41^* & \\ 
\hline
\multirow{2}{*}{Chewie-day2} & acc & 72.29^* & x  & & 57.17^* & 60.95^* & \\ & delta-acc & 72.29^* & x  & & 57.17^* & 60.95^* & \\
\hline
\multirow{2}{*}{Mihi-day1} & acc & 63.64^* & x  & & 59.50^* & 70.48^* & \\ & delta-acc & 63.64^* & x  & & 59.50^* & 70.48^* & \\
\hline
\multirow{2}{*}{Mihi-day2}  & acc & 61.49^* & x  & & 60.82^* & 64.35^* & \\ & delta-acc & 61.49^* & x  & & 60.82^* & 64.35^* & \\ \hline
\end{tabular}
\begin{tabular}{llcccccc}

            & & supervised & VAE & pi-VAE & BYOL & MYOW & Ours \\\hline
\multirow{2}{*}{Chewie-day1} & MSE & x & x  & x & x & x & \\ & CE & x & x  & x & x & x & \\ 
\hline
\multirow{2}{*}{Chewie-day2} & MSE & x & x  & x & x & x & \\ & CE & x & x  & x & x & x & \\ 
\hline
\multirow{2}{*}{Mihi-day1} & MSE & x & x  & x & x & x & \\ & CE & x & x  & x & x & x & \\ 
\hline
\multirow{2}{*}{Mihi-day2} & MSE & x & x  & x & x & x & \\ & CE & x & x  & x & x & x & \\ 
\hline
\end{tabular}
\end{table}




==> text/decoding2.tex <==




\begin{table}[h]
\centering
\caption{Accuracy (in \%) for classification on neural datasets. Here * means that the data is copied from MYOW and is subject to change.}
\label{table: classification}
\begin{tabular}{llcccccc}

            & & supervised & VAE & pi-VAE & BYOL & MYOW & Ours \\\hline
\multirow{2}{*}{Chewie-day1} & acc & 63.29^* & x  & & 63.80^* & 70.41^* & \\ & delta-acc & 63.29^* & x  & & 63.80^* & 70.41^* & \\ 
\hline
\multirow{2}{*}{Chewie-day2} & acc & 72.29^* & x  & & 57.17^* & 60.95^* & \\ & delta-acc & 72.29^* & x  & & 57.17^* & 60.95^* & \\
\hline
\multirow{2}{*}{Mihi-day1} & acc & 63.64^* & x  & & 59.50^* & 70.48^* & \\ & delta-acc & 63.64^* & x  & & 59.50^* & 70.48^* & \\
\hline
\multirow{2}{*}{Mihi-day2}  & acc & 61.49^* & x  & & 60.82^* & 64.35^* & \\ & delta-acc & 61.49^* & x  & & 60.82^* & 64.35^* & \\ \hline
\end{tabular}
\end{table}



\begin{table}[h]
\centering
\caption{Accuracy (in \%) for position classification on neural datasets.}
\label{table: classification}
\begin{tabular}{llcccccc}

            & & supervised & VAE & pi-VAE & BYOL & MYOW & Ours \\\hline
\multirow{2}{*}{Chewie-day1} & MSE & x & x  & x & x & x & \\ & CE & x & x  & x & x & x & \\ 
\hline
\multirow{2}{*}{Chewie-day2} & MSE & x & x  & x & x & x & \\ & CE & x & x  & x & x & x & \\ 
\hline
\multirow{2}{*}{Mihi-day1} & MSE & x & x  & x & x & x & \\ & CE & x & x  & x & x & x & \\ 
\hline
\multirow{2}{*}{Mihi-day2} & MSE & x & x  & x & x & x & \\ & CE & x & x  & x & x & x & \\ 
\hline
\end{tabular}
\end{table}


==> text/intro.tex <==

\section{Introduction}
In the brain, the coordinated action of groups of neurons is responsible for encoding sensory inputs, generating movements, and everything in between.
%Understanding how neural circuits and populations of neurons encode information 
Although neurons are powerful, the activity of individual neurons is often highly variable, even in constrained settings \cite{de2020large,talebi2012natural,shadlen1998variable,kandel2000principles,hubel1959receptive,vinje2000sparse}. 
As a result, it is challenging to decode complex behavior from the activity of a population of neurons given only the raw records of their spike times \cite{pandarinath2018latent}. 
Remarkably, however, even when the individual responses of neurons vary, their population-level responses, 
%which are considered to be the basis of sensation, perception, cognition, and behavior, 
remain stable (to some extent) \cite{gallego2020long,afshar2011single,pandarinath2018inferring}. 
This suggests that by learning representations of neural activity that can reveal these underlying stable latent factors, we could build more robust decoders for information encoded in the brain and also gain insights into individual differences across task learning. 


With the rapid growth of deep learning, there has been a great deal of interest in applying these methods to extract representations of neural activity that reveal underlying links to behavior or decision making \cite{zhou2020learning,prince2021parallel,keshtkaranlarge,ye2021representation,pandarinath2018inferring, azabou2021mine,loaiza2019deep}. The success of such approaches often grants insights into how neural circuits work to encode their inputs and drive decisions. However, without labels, learning latent spaces that can appropriately reveal and {\em disentangle different sources of variability} is still a major challenge \cite{locatello2019challenging,higgins2018towards}.
%Striking the right balance between interpretability, disentanglement, and reconstruction accuracy is not trivial. 
Moving forward, we need new unsupervised tools to decompose the latent factors that drive neural population activity. 

%\eva{compare w sequential models like lfads}


Here, we develop a novel self-supervised approach for generative modeling of neural activity called {\em Swap-VAE}. Our approach is loosely inspired by methods used in computer vision that aim to decompose images into their {\em content} and {\em style} \cite{mathieu2016disentangling,zhang2018style,huang2017arbitrary,zhang2018multi,karras2019style}: the representation of the content should give us the abstract ``gist'' of the image (what it is), and the style components are needed to create a realistic image (or, equivalently, they capture the variation in images with the same content). To map this idea onto the decomposition of brain states, consider the execution of movements and their representation within the the brain (Figure~\ref{fig-overview}, Right). The content in this case may be {\em knowing where to go} (target location) and the style would be the {\em exact execution of the movement} (the movement dynamic). We ask whether the neural representation of movement can be disentangled into these components using our proposed conceptual framework.

To build the content space, our goal is to minimize an instance-specific alignment loss that effectively penalizes the deviation between {\em transformed views} of the input in the latent space of the encoder. In other words, we apply a variety of transformations to the input data in an effort to learn the consistent "truth" that persists despite manipulation.  These transformed (or augmented) views are created by dropping out neurons and jittering samples in time, which intuitively should lead the network to a representation that maintains both temporal consistency and invariance to the specific neurons used to represent the neural state.  In addition to this alignment loss, we use a separate set of latent variables to reconstruct the original inputs using a regularized variational autoencoder ($\beta$-VAE \cite{higgins2016beta,burgess2018understanding}). To further encourage disentanglement, we introduce a novel latent space augmentation called {\em BlockSwap}, where we swap the content components of two examples and ask the network to predict the original view. We show that through combining our self-supervised alignment loss with a generative model, we can build good representations that disentangle latent factors underlying neural population activity. 

We apply our method to synthetic data and non-human primate (NHP) reaching datasets from two different individuals (using the same datasets as in \cite{azabou2021mine} from \cite{dyer2017cryptography}). To quantify the disentanglement of our representations of these data, we compute a number of measures of representation quality and also compute linear decoding accuracies across both spaces to test whether more information about the target (what) and time (how) are encoded in the two different spaces. We show that by using our approach, we can effectively disentangle the behavior and dynamics of movement without any labels. Our model strikes a nice balance between both view-invariant representation and generation.
 
Our specific contributions are as follows:  
\vspace{-1mm}
\begin{itemize}
     \item In Section~\ref{sec:methods}, we propose a generative method, \alg\hspace{-1mm}, that can both (i) learn a representation of neural activities that reveal meaningful and interpretable latent factors and (ii) generate realistic neural activities. %Our proposed method may reveal the relationship between the brain and behavior.
     \vspace{-0.4mm}
     \item In Section~\ref{sec:blockswap}, we propose a novel latent representation augmentation procedure called {\em BlockSwap} which swaps variables in the latent space to improve disentanglement.
     \vspace{-0.4mm}
     \item In Section~\ref{sec:metrics}, we introduce metrics to quantify the disentanglement of our representations of behavior and apply them to neural datasets from different non-human primates (Section~\ref{sec:experiments}) to gain insights into the link between neural activity and behavior. 
     \vspace{-2mm}
     %The proposed metrics reveal the differences of brain activities when being used to compare the neural activities of monkeys that perform tasks in different laboratory settings.
     %These measures, when applied to our model's outputs, can provide insights into how entangled direction and movement speed are in the brains of different individuals. 
\end{itemize}


\begin{figure*}
\centering
    \includegraphics[width=0.91\textwidth]{imgs/overview_fig_ran_v2.jpg}
    \caption{\footnotesize{\em Overview of approach.} The model's latent variables are partitioned into a content space and a style space. An instance-specific loss is applied to the content representations of augmented views of a brain state (shifting in time and dropping out neurons) to encourage alignment, while views are reconstructed at the output of the decoder using both parts of the latent space. To further enhance the clustering in the content space, we introduce {\em BlockSwap}: two augmented views are projected through the encoder and in the content space their representations are swapped before being passed through the decoder. To the right, we show an example of applying this approach to disentangle the neural representation of movement.}
    \vspace{-3mm}
    \label{fig-overview}
\end{figure*}

==> text/oldstuff.tex <==
%We build on this SSL framework and show how their local instance-specific alignment objective can be coupled with a generative model to achieve both good representation quality and disentanglement while also removing the need for a dual network approach.
%Specifically, BYOL tries to solve the following objective:
%Recently there are a lot of progress on the development of self-supervised learning methods \cite{misra2020self,chen2020simple,he2020momentum,grill2020bootstrap,chen2020exploring,caron2020unsupervised}.They can be roughly category to two types of methods: contrastive-based and clustering-based. Contrastive learning based methods utilize both positive examples and negative examples, and a large amount of negative examples is key for contrastive methods to perform well \cite{chen2020simple,he2020momentum}. While clustering based methods still require positive examples, they do not require negative example directly. Some clustering methods require a large amount of positive examples while learning \cite{caron2020unsupervised}, while some do not \cite{grill2020bootstrap}. There are hypothesis show that in some methods the cluster center serves as the implicit negative example prototype \cite{chen2020exploring}.
%Then, they show how a nearest-neighbor based strategy for incorporating nonlocal brain states as positive examples could be used to boost the neural decoding accuracies significantly, and deliver performance above supervised methods. 

%We build on, and in some ways simplify, this framework and show how their instance-specific alignment objective can be coupled with a generative model to achieve both good representation quality and disentanglement while also removing the need for a dual network approach. %We show how our BlockSwap augmentation and loss can be used to improve decoding accuracy and disentanglement even further.


% \rliu{The current section 2 is a little bit awkward since it kind of both introduce related works and background. IMHO, background should include only 1) neural data 2) VAE, beta-VAE. related work should include 1) VAE-ish works for neural activities. 2) The content/style separation works in computer vision (we motivate our work based on those). 3) SSL. What about we break down this section, make background real short, and have a related work section before the conclusion?}




==> text/relatedwork.tex <==
\section{Related Work}

\paragraph{Representation learning for neural activity.}

%Recently, a number of approaches have been proposed to build representations of neural activities
%\cite{zhou2020learning,prince2021parallel,keshtkaranlarge,ye2021representation,pandarinath2018inferring, azabou2021mine}. Methods can be generally categorized into models that use sequential backbones (like Lfads, NDT) and those that treat brain state information across different time points as independent samples (Pi-VAE, MYOW, our model). 




%\rliu{Sure we can add this in related work section. I just think it is strong.}

\vspace{-3mm}
\paragraph{Connection and innovations over generative models in computer vision and general ML.}
There are a lot of generative models in computer vision field. Among them, there are many approaches that consider a content/style separation decomposition like what we use in our approach \cite{zhang2018style,park2020swapping,zhang2018separating}. In this literature, style/content swapping is often used, but usually through the use of labels \cite{lee2018diverse}.

More recently, models have combined generation and self-supervision. InfoGAN-CR \cite{lin2020infogan} builds on InfoGAN and used a contrastive regularizer to perform better disentanglement. Our model is different from all of them (to the best of our knowledge) since our model use the augmentations and the corresponding positive views clustering in the content space. 

%In almost all self-supervised learning methods, different augmentations (views) are critical for learning. 
%While contrastive based methods focus on comparing different views and clustering based methods focus on cluster different views. [Carefully check if there is any work that does not use different views] In works that investigate different pretext tasks \cite{}, they analyzed that different augmentations let the model to learn in-variants across images.

%Recent self-supervised learning methods showed the importance of data augmentations. There are two types of self-supervised learning methods based on data augmentations: invariance ones that seeks to cluster the positive views and covariance ones that seeks to predict the properties of data augmentations. Our methods use both of them.










